An approximation algorithm for zero forcing

We give an algorithm that finds a zero forcing set which approximates the optimal size by a factor of $\text{pw}(G)+1$, where $\text{pw}(G)$ is the pathwidth of $G$. Starting from a path decomposition, the algorithm runs in $O(nm)$ time, where $n$ and $m$ are the order and size of the graph, respectively. As a corollary, we obtain a new upper bound on the zero forcing number in terms of the fort number and the pathwidth. The algorithm is based on a correspondence between zero forcing sets and forcing arc sets. This correspondence leads to a new bound on the zero forcing number in terms of vertex cuts, and to new, short proofs for known bounds on the zero forcing number.

==> figures/cut-enlighten.tex <==

\begin{figure}
\centering
\begin{minipage}[h]{.45\textwidth}
\begin{tikzpicture}[shorten >=1pt,->]
\tikzstyle{solid}=[circle, fill, inner sep=1.5pt]
\tikzstyle{empty}=[circle,draw=black, inner sep=1.5pt]
% \tikzstyle{dashed arrow}=[densely dotted, -stealth]
% \tikzstyle{bold}=[line width=1.5pt, densely dashed]
\tikzstyle{bold}=[->, line width=1.5pt]
\tikzstyle{dashed snake} = [->, dashed, line width = 1.3pt]
\tikzstyle{edge}=[-]
\tikzstyle{vertex}=[]
% \node at (3.5, -3.8) {$u_2$};
% \node[empty] (u4) at (4.8, -2) {};
% \draw[edge] (-21) -- (u1);


% box for C
\draw[very thick,dashed] (-.7, -.6)rectangle(.7, 4.4) ;
\node at (0, 4.7) {$C$};
% box for G1
\draw[dashed] (-3, -.4)rectangle(.5, 4.2) ;
\node at (-1.5, 4.5) {$G_1$};
% box for G2
\draw[dashed] (-.5, -.2)rectangle(3, 4.) ;
\node at (1.5, 4.5) {$G_2$};

\foreach \i in {0,...,3}{
    \node[solid] (\i0) at (0,    \i*0.9+.6) {};
    \node[solid] (\i1) at (-1.4,   \i*0.9+.6) {};
    \node[solid] (\i3) at (-2.7,  \i*0.9+.6) {};
    
    \node[solid] (\i2) at (1.4,    \i*0.9+.6) {};
    \node[solid] (\i4) at (2.7, \i*0.9+.6) {};
    
    \draw[bold] (\i0) -- (\i1);
    \draw[bold] (\i2) -- (\i0);
    \draw[dashed snake] (\i1) -- (\i3);
    \draw[dashed snake] (\i4) -- (\i2);
}
\node at (0, 3.6) {$v_0$};
\node at (-1.4, 3*0.9+0.6+0.3) {$v_1$};
\node at (-1.4, 0.2) {$v_{s-1}$};
\node at (0, 1.8) {$v_s$};
\draw[edge] (0, 1*0.9+0.6) -- (-1.4, 0*0.9+0.6);
\end{tikzpicture}
\end{minipage}
\begin{minipage}[h]{.45\textwidth}
\begin{tikzpicture}[shorten >=1pt,->]
\tikzstyle{solid}=[circle, fill, inner sep=1.5pt]
\tikzstyle{empty}=[circle,draw=black, inner sep=1.5pt]
\tikzstyle{bold}=[->, line width=1.5pt]
\tikzstyle{dashed snake} = [->, dashed, line width = 1.3pt]
\tikzstyle{edge}=[-]
\tikzstyle{vertex}=[]

% box for C
\draw[very thick,dashed] (-.7, -.6)rectangle(.7, 4.4) ;
\node at (0, 4.7) {$C$};
% box for G1
\draw[dashed] (-3, -.4)rectangle(.5, 4.2) ;
\node at (-1.5, 4.5) {$G_1$};
% box for G2
\draw[dashed] (-.5, -.2)rectangle(3, 4.) ;
\node at (1.5, 4.5) {$G_2$};

\foreach \i in {0,...,3}{
    \node[solid] (\i0) at (0,    \i*0.9+.6) {};
    \node[solid] (\i1) at (-1.4,   \i*0.9+.6) {};
    \node[solid] (\i3) at (-2.7,  \i*0.9+.6) {};
    
    \node[solid] (\i2) at (1.4,    \i*0.9+.6) {};
    \node[solid] (\i4) at (2.7, \i*0.9+.6) {};
    
    \draw[bold] (\i0) -- (\i1);
    \draw[bold] (\i2) -- (\i0);
    \draw[dashed snake] (\i1) -- (\i3);
    \draw[dashed snake] (\i4) -- (\i2);
}
\node at (0, 3.6) {$v_0$};
\node at (-1.4, 2*0.9+0.6+0.3) {$v_1$};
\draw[edge] (0, 3*0.9+0.6) -- (-1.4, 2*0.9+0.6);
\node at (0, .2) {$v_{s-1}$};
\node at (0, 1.8) {$v_s$};
\draw[edge] (0, 1*0.9+0.6) -- (0, 0*0.9+0.6);
\end{tikzpicture}
\end{minipage}
\caption{An illustration for the proof of Proposition~\ref{prop:cut}, where the arrows indicate forcing arc set $A_1$ for $G_1$ and $\overleftarrow{A_2}$ for $G_2$. 
There may be other sources that are not in the cut; we omit them for clarity. 
The two figures are for possible cases of $v_1$ and $v_{s-1}$ (that is, whether or not in $C$), where $v_0$ and $v_s$ are positioned the same. The edge $v_0v_1$ either is an arc or not, but $(v_{s-1},v_s)\notin A$ necessarily.}
\label{fig:cut-enlighten}
\end{figure}




==> figures/non-2-parallel_paths.tex <==
\begin{figure}
  		\centering
		\begin{tikzpicture}[shorten >=1pt,->]
 		%\tikzstyle{vertex}=[circle,draw=black!60,minimum size=12pt,inner sep=2pt]
		\tikzstyle{w}=[circle, draw=black,minimum size=12pt,inner sep=2pt]
		\tikzstyle{b}=[circle, draw=black,fill=black, minimum size=12pt, text=white, inner sep=2pt]
 		\node[b] (1) at (0,0) {$\pmb{v_1} $};
 		\node[b] (2) at (2,0) {$\pmb{v_{i}}$};
 		\node[w] (3) at (4,0) {$v_{j}$};
 		\node[w] (4) at (6,0) {$v_m$};
  
  		\node[b] (5) at (0,-1.5) {$\pmb{u_1}$};
  		\node[b] (6) at (2,-1.5) {$\pmb{u_{i'}}$};
  		\node[w] (7) at (4,-1.5) {$u_{j'}$};
 		\node[w] (8) at (6,-1.5) {$u_{n}$};
  
		\draw[densely dotted] (1)--(2)--(3)--(4)--cycle ;
  		\draw[densely dotted] (5)--(6)--(7)--(8)--cycle ;
		
		\draw (1) --(5) -- cycle;
		\draw (4) --(8) -- cycle;
		\draw (3) -- (6) -- cycle;
		\draw (2) --(7) -- cycle;
  
		\end{tikzpicture}
		\caption{A graph is not of two parallel paths}
	\label{fig:boat}
\end{figure}

==> figures/ppw-wo-chaintwist.tex <==
\begin{figure}
	\centering
	\begin{subfigure}{.5\textwidth}
  		\centering
		\begin{tikzpicture}[shorten >=1pt,->]
 		\tikzstyle{vertex}=[circle,draw=black!60,minimum size=12pt,inner sep=2pt]
 		\node[vertex] (v11) at (0,0) {$u_{1}$};
 		\node[vertex] (u1) at (2,0) {$u_{i}$};
 		\node[vertex] (w1) at (4,0) {$u_{j}$};
 		\node[vertex] (v14) at (6,0) {$u_{l}$};
  
  		\node[vertex] (v21) at (0,-1.5) {$v_{1}$};
  		\node[vertex] (u2) at (2,-1.5) {$v_{i'}$};
  		\node[vertex] (w2) at (4,-1.5) {$v_{j'}$};
 		\node[vertex] (v24) at (6,-1.5) {$v_{m}$};
  
  		\node[vertex] (v31) at (0,-3) {$w_{1}$};
  		\node[vertex] (u3) at (2,-3) {$w_{i''}$};
  		\node[vertex] (w3) at (4,-3) {$w_{j''}$};
  		\node[vertex] (v34) at (6,-3) {$w_{n}$};
  
  
  		\draw[densely dotted] (v11) -- (u1) -- (w1) -- (v14) -- cycle;
  		\draw[densely dotted] (v21) -- (u2) -- (w2) -- (v24) -- cycle;
  		\draw[densely dotted] (v31) -- (u3) -- (w3) -- (v34) -- cycle;
  
  		\draw (u1)--(w2)--cycle; 
  		\draw (u2)--(w3)--cycle;
  		\draw (u3)--(w1)--cycle; 
		\end{tikzpicture}
		\caption{A path partition with indexing\\ that has a chain twist}
		\label{exampleWrongIndex}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
 		\centering
		\begin{tikzpicture}[shorten >=1pt,->]
 		\tikzstyle{vertex}=[circle,draw=black!60,minimum size=12pt,inner sep=2pt]
 		\node[vertex] (v11) at (0,0) {$u_{1}$};
 		\node[vertex] (u1) at (2,0) {$u_{i}$};
 		\node[vertex] (w1) at (4,0) {$u_{j}$};
 		\node[vertex] (v14) at (6,0) {$u_{l}$};
  
  		\node[vertex] (v21) at (6,-1.5) {$v_{1}$};
  		\node[vertex] (w2) at (2,-1.5) {$v_{i'}$};
  		\node[vertex] (u2) at (4,-1.5) {$v_{j'}$};
 		\node[vertex] (v24) at (0,-1.5) {$v_{m}$};
  
  		\node[vertex] (v31) at (0,-3) {$w_{1}$};
  		\node[vertex] (u3) at (2,-3) {$w_{i''}$};
  		\node[vertex] (w3) at (4,-3) {$w_{j''}$};
  		\node[vertex] (v34) at (6,-3) {$w_{n}$};

 		\draw[densely dotted] (v11) -- (u1) -- (w1) -- (v14) -- cycle;
  		\draw[densely dotted] (v24) -- (w2) -- (u2)-- (v21) -- cycle;
  		\draw[densely dotted] (v31) -- (u3) -- (w3) -- (v34) -- cycle;
  
 		\draw (u1)--(w2)--cycle; 
 		\draw (u2)--(w3)--cycle;
  		\draw (u3)--(w1)--cycle; 
		\end{tikzpicture}
		\caption{A path partition with indexing\\ does not have a chain twist} \label{exampleRightIndex} 
		\end{subfigure}
	\caption{Different indexed path partition on the same graph }
	\label{fig:iipp}
\end{figure}
